ATPPNet: Attention based Temporal Point cloud Prediction Network

Point cloud prediction is an important yet challenging task in the field of autonomous driving. The goal is to predict future point cloud sequences that maintain object structures while accurately representing their temporal motion. These predicted point clouds help in other subsequent tasks like object trajectory estimation for collision avoidance or estimating locations with the least odometry drift. In this work, we present ATPPNet, a novel architecture that predicts future point cloud sequences given a sequence of previous time step point clouds obtained with LiDAR sensor. ATPPNet leverages Conv-LSTM along with channel-wise and spatial attention dually complemented by a 3D-CNN branch for extracting an enhanced spatio-temporal context to recover high quality fidel predictions of future point clouds. We conduct extensive experiments on publicly available datasets and report impressive performance outperforming the existing methods. We also conduct a thorough ablative study of the proposed architecture and provide an application study that highlights the potential of our model for tasks like odometry estimation.

==> relatedworks.tex <==
\section{Related works}

\subsection{Static point cloud processing }
Static point clouds are an unordered set of points that are invariant to the permutations. As a result, convolution operations that work on images cannot be applied directly on point clouds. Multi-view methods like \cite{su15mvcnn, yu2018multi, yang2019learning} project the unstructured point cloud to $2D$ images and then extract view-wise features. These features are then fused together and used for applications like classification, detection and tracking. Volumetric-based methods like \cite{maturana2015voxnet, riegler2017octnet, wang2017cnn} convert the point clouds into $3D$ volumetric representations like voxels and then apply $3D$ convolutional operations to perform the downstream tasks. Pointwise MLP methods models each points in a point cloud independently and then aggregates a global feature by using a symmetric aggregation function. PointNet \cite{qi2017pointnet} takes a pointcloud as input and learns pointwise features independently using several MLP layers. PointNet++ \cite{qi2017pointnet++} is based on PointNet and is a hierarchical network than can capture fine geometric structures. Pointasnl \cite{yan2020pointasnl} can capture the local and long range dependencies of points sampled by the Furthest Point Sampling (FPS) algorithm by utilizing an Adaptive Sampling (AS) module to adaptively adjust the coordinates and features of points sampled by the Furthest Point Sampling (FPS) algorithm.

\subsection{Sequential point cloud processing }
One of the main challenges in point cloud prediction is modelling the spatio-temporal features of a sequence of point clouds and use them to solve tasks related to autonomous systems and robotics. Liu et al. proposed FlowNet3D \cite{liu2019flownet3d} to estimate the $3D$ motion field between two point clouds. Lu et al. proposed Pointinet \cite{lu2021pointinet} to interpolate intermediate frames between two LiDAR point clouds. Fast and Furious \cite{luo2018fast} by Luo et al. performs detection, tracking and motion forecasting on a sequence of bird’s eye view representation of the 3D world. MotionNet \cite{wu2020motionnet} by Wu et al. processes a sequence of point clouds using spatio-temporal pyramid network and outputs a bird’s eye view (BEV) map, which encodes the object category and motion information in each grid cell.


\subsection{Point cloud Prediction} 
\subsubsection{Point Clouds methods}
Fan et al. proposed PointRNN \cite{fan2019pointrnn} that predicts the future sequences of unordered point clouds by adopting spatio-temporally local correlations to model the point features and states. MoNet \cite{lu2021monet} by Lu et al. combines motion features with content features and processes them using a novel recurrent neural network to generate future sequences of point clouds. Deng et al. \cite{deng2020temporal} reformulates the task of pointcloud prediction as a motion prediction problem where they learn the dynamics of the scene using flow embedding and outputs a motion vector for each point in the current frame which is then added to these points to get the point cloud for the next frame. All of these works are based on the $3D$ point clouds and considers only a limited number of points. 

\subsubsection{Range image based methods}
Weng et al. SPFNet \cite{spf2} adopted an encoder-decoder architecture to predict future point clouds. They explored using point based encoders (PointNet \cite{qi2017pointnet}) and range image based methods and concluded that projecting the point clouds into range images and then predicting the range images performs better than directly predicting point clouds. Based on SPFNet, Weng et al. proposed S2Net \cite{weng2022s2net} which uses a pyramid-LSTM module along with a conditional variational LSTM to predict stochastic future point clouds.
TCNet by Mersch et al. \cite{mersch2022self} projected the past point clouds as $2D$ range images and concatenated them to generate $3D$ tensors. $3D$ spatio-temporal CNNs with skip-connections and circular padding are then used to process this input $3D$ tensor and generate range images for future timesteps. Luo et al. proposed PCPNet \cite{pcpnet} that leverages the self-attention mechanism of Transformers by compressing the range images along the height and width to generate sentence like features and use a semantic-based loss function to generate the future sequences.
Manttari et al. \cite{manttari2020interpreting} presented a study comparing $3D$ CNN and ConvLSTMs and came to the conclusion that the $3D$ CNN models concentrates on shorter events in the input sequence, and places its spatial focus on fewer, contiguous areas whereas ConvLSTMs focus more on smaller areas on several objects in the scene. 
